Nonlinear model reduction of dynamical power grid models using quadratization and balanced truncation

In this work, we present a nonlinear model reduction approach for reducing two commonly used nonlinear dynamical models of power grids: the effective network (EN) model and the synchronous motor (SM) model. Such models are essential in real-time security assessments of power grids. However, as power grids are often large-scale, it is necessary to reduce the models in order to utilize them in real-time. We reformulate the nonlinear power grid models as quadratic systems and reduce them using balanced truncation based on approximations of the reachability and observability Gramians. Finally, we present examples involving numerical simulation of reduced EN and SM models of the IEEE 57 bus and IEEE 118 bus systems.

==> csc-bibfiles/README <==
==The files==
mor.bib:
Contains anything model order reduction related including
applications. Papers on helper problems like solvers for matrix
Lyapunov equations do NOT belong here.

software.bib:
This is the resource for anything software related. Mostly manuals and
WWW references go here.

csc.bib:
Everything else goes in here.


Note that these files are supposed to be disjoint!

All files are located in the group SVN under
http://svncsc.mpi-magdeburg.mpg.de/repos/mpcsc/pubs/bibfiles/

The formating of the files is the one produced by emacs in
BibTeX-mode. Use the emacs menu 
   Bibtex-Edit -> Operation on Buffer ->

   	       -> Validate Entries
	       -> Sort Entries
	       -> Reformat Entries

to ensure you have the proper formatting. 
If you can not use emacs:
 - Sorting is performed according to the bibtex keys.
 - try to adapt the formating found in the other entries.
 
JabRef can be used to do the sorting, but will destroy the formating
of the entries. 

MOST IMPORTANTLY:
When checking in your changes to the SVN repository, please make sure 
you give a meaningful log message telling which entries have been added, 
upated or whatever. Since not everyone is using emacs the formatting of the 
entries and their sorting will change depending on the editor and it will
be almost impossible to keep track of the actual changes otherwise.

==Comparing multiple bib-files==
If you need to compare (e.g. to merge them) two bibfiles.
It is a good idea to use the same editor (preferably emacs using the
above) to ensure the same sorting and formating in both files and then
use a graphical diff tool (e.g. mgdiff, kdiff3, xxdiff,...) to check
for the differences. Most of those tools can perform merge operations
already. Currently (summer 2011) these tools are not automatically
installed on our computers, so you need to ask the IT to install one
on yours. 

==Naming schemes and entry format rules==

===Publication types===
When in doubt about a publication type try to discuss it here and on
the group mailing list.

===Preprint handling==
Enter a new preprint as TechReport with all the data as on the corresponding
Preprint server.
Add 
type = {Preprint}

Once submitted add:
 note = {Submitted to }
and change this to
 note = {To appear in }
on acceptance. 

When the final paper has appeared add it as a separate entry with own
bibtex key. 
Then remove the TechReport from the database!

=== Other Technical reports==
Entries for technical report should have a type entry to distinguish them from submitted preprints:

type = {Technical reports}

or 

a more detailed description, e.g.

type = {SLICOT Working Note},


ArXiv entries should be written as TechReport following the example in the CSC Wiki


===BibTeX Keys===
Bibtex keys for the entries are formed from the authors name(s) and
the year of publication as in 

  3 leading characters of first authors last name (Xxx)
 +1 leading character of second and third atuhros last names (YZ)
 +year of publication as 2 digits (11)
 +1 additional character for counting if the previous is non-unique

In the mor.bib file an additional leading mor is added.
 
examples:
Xxx08, XxxYZ10, XxxYZ10a, XxxYZ10b
examples mor.bib:
morXxx08, morXxxYZ10, morXxxYZ10a, morXxxYZ10b

===author fields===
First names are abbreviated by 1character. In case of multiple first
names, these are separated by a single empty space or secured space (~).
Multiple authors are separated by an and.

example:
author = {J. F. Kennedy and F. D. Roosevelt}
author = {Kennedy, J.~F. and Roosevelt, F.~D.}
author = {M. {Van~Barel}}

===booktitle fields===
Since Bibtex Strings and standard entries can not be combined be sure
to meet the String format and add the special information such as , e.g.,
years, or numbers in case of conference Proceedings

===publisher, journal, month fields===
Make sure you check the list of BibTex Strings and use existing
strings here or add new ones where necessary. 

Follow the list of the AMS for Mathematical reviews available at: 
 http://www.ams.org/msnhtml/serials.pdf
for new entries

Use three-letter abbreviations without quotes for months like
month = mar,
month = jun,

===pages===
Page ranges should be given with double dashes

example:
 pages = {102--110}

===German Umlaut and other special characters===
Always use LaTeX transcription for any of these characters to avoid
problems with differing file encodings. 
examples 
 ä -> \"{a}
 ß -> {\ss}


==> tex/backup/numerical_example_output_error.tex <==
\newcommand{\outputerrorplot}[4]{
\begin{tikzpicture}
\begin{axis}[plot_style,
	xlabel={{$n_r$}},
	ylabel={{$L^2$-norm of the output error}},
	ymode=log]

% Add vertical line
\addplot[thick, forget plot] coordinates { (#4, 1e-16) (#4, 1e16) };

% Add BT(i) plots
\foreach \i in {1, 3, ..., #3}{
	\addplot+[ultra thick, mark=otimes] table[x index=0, y 		index=1]{./results/output_error/output_error_#1_#2_bt\i.dat};
	\iflegendenabled\addlegendentryexpanded{BT(\i)};\fi
}

% Add POT plots
\addplot+[ultra thick, mark=otimes] table[x index=0, y index=1]{./results/output_error/output_error_#1_#2_pod.dat};
\iflegendenabled\addlegendentry{POD};\fi

%    \foreach \i in {1,...,10}
%      \addplot[smooth, dashed, ultra thick, blue!50!white] table [x index=0, y index=\i]{results/fom_test_angles.txt};
\end{axis}
\end{tikzpicture}
}

==> tex/backup/numerical_example_pti_error.tex <==
\newcommand{\ptierrorplot}[4]{
\begin{tikzpicture}
\begin{axis}[plot_style,
	xlabel={{$n_r$}},
	ylabel={{$L^2$-norm of the PTI error}},
	ymode=log]

% Add vertical line
\addplot[thick, forget plot] coordinates { (#4, 1e-16) (#4, 1e16) };

% Add BT(i) plots
\foreach \i in {1, 3, ..., #3}{
	\addplot+[ultra thick, mark=otimes] table[x index=0, y 		index=3]{./results/output_error/output_error_#1_#2_bt\i.dat};
	\iflegendenabled\addlegendentryexpanded{BT(\i)};\fi
}

% Add POT plots
\addplot+[ultra thick, mark=otimes] table[x index=0, y index=3]{./results/output_error/output_error_#1_#2_pod.dat};
\iflegendenabled\addlegendentry{POD};\fi

%    \foreach \i in {1,...,10}
%      \addplot[smooth, dashed, ultra thick, blue!50!white] table [x index=0, y index=\i]{results/fom_test_angles.txt};
\end{axis}
\end{tikzpicture}
}

==> tex/figures/Recycle Bin/numerical_example_pti_error.tex <==
\newcommand{\ptierrorplot}[5]{
\begin{tikzpicture}
\begin{axis}[plot_style,
	xmin=1,
	xmax={{2*#5}},
	xlabel={{$n_r$}},
	ylabel={{$L^2$-norm of the PTI error}},
	xtick={#4},
	ymode=log,]

% Add vertical line
\addplot[thick, forget plot] coordinates { (#5, 1e-16) (#5, 1e16) };

% Add BT(i) plots
\foreach \i in {1, 3, ..., #3}{
	\addplot+[ultra thick, mark=otimes] table[x index=0, y 		index=3]{./results/comparison_with_pod/output_error_#1_#2_bt\i.dat};
	\iflegendenabled\addlegendentryexpanded{BT(\i)};\fi
}

% Add POD plots
\addplot+[ultra thick, mark=otimes] table[x index=0, y index=3]{./results/comparison_with_pod/output_error_#1_#2_pod.dat};
\iflegendenabled\addlegendentry{POD};\fi
\end{axis}
\end{tikzpicture}
}

==> tex/info.tex <==
\articletype{Methods}

\author*[1]{Tobias K. S. Ritschel}
\author[2]{Frances Wei{\ss}}
\author[2]{Manuel Baumann}
\author[2]{Sara Grundel}
\runningauthor{Ritschel et al.}
\affil[1]{Max Planck Institute for Dynamics of Complex Technical Systems \texttt{ritschel@mpi-magdeburg.mpg.de}}
\affil[2]{Max Planck Institute for Dynamics of Complex Technical Systems \texttt{grundel@mpi-magdeburg.mpg.de}}
\title{Nonlinear model reduction\\of dynamical power grid models\\using quadratization and balanced truncation}
\runningtitle{Nonlinear balanced truncation of dynamical power grid models}
%\subtitle{...}
\abstract{\input{tex/abstract}}
\keywords{Nonlinear model reduction,
	balanced truncation,
	dynamical power grid models,
	quadratic systems}
%\classification[PACS]{...}
%\communicated{...}
%\dedication{...}
%\received{...}
%\accepted{...}
\journalname{at - Automatisierungstechnik}
\journalyear{2020}
%\journalvolume{..}
%\journalissue{..}
\startpage{1}
%\aop
%\DOI{...}

==> tex/numerical_example_basic_comparison.tex <==
% CREATE PLOTS OF L2 ERRORS
\begin{figure*}
	\subfloat[Output errors (EN model).\label{fig:output_error_en_case57}]{%
		\centering
		\legendenabledtrue % Enable legend
		\outputerrorplot{en}{case57}{1}{7}{7}{$L^2$-norm of the output error}{1e-18}{1e0} % arg. 6: 1 = L2, 2 = Linf
	}~
	%
	\subfloat[Output errors (SM model).\label{fig:output_error:sm:case57}]{%
		\centering
		\legendenabledfalse % Disable legend
		\outputerrorplot{sm}{case57}{1}{7}{57}{$L^2$-norm of the output error}{1e-18}{1e0} % arg. 6: 1 = L2, 2 = Linf
	}
	\\[10pt]
	\subfloat[Pythagorean trigonometric identity errors (EN model).\label{fig:pti_error_en_case57}]{%
		\centering
		\legendenabledfalse % Disable legend
		\outputerrorplot{en}{case57}{3}{7}{7}{$L^2$-norm of the PTI error}{1e-18}{1e0} % arg. 6: 3 = L2, 4 = Linf
	}~
	%
	\subfloat[Pythagorean trigonometric identity errors (SM model).\label{fig:pti_error_sm_case57}]{%
		\centering
		\legendenabledfalse % Disable legend
		\outputerrorplot{sm}{case57}{3}{7}{57}{$L^2$-norm of the PTI error}{1e-18}{1e0} % arg. 6: 3 = L2, 4 = Linf
	}
	\caption{$L^2$ error of the ROM predictions.}
\end{figure*}

==> tex/qmor_pod.tex <==
$X = \begin{bmatrix} x(t_1) & \cdots & x(t_M) \end{bmatrix}$

$X = U\Sigma V^T$

$\mathcal W = \mathcal V = U_r$

\begin{remark}
	we use Matlab's \texttt{ode45} routine with $M$ prespecified time points to generate the snapshots. Consequently, as \texttt{ode45} uses adaptive time step sizes, the snapshot matrix, $X$, does not necessarily include all time steps.
\end{remark}

==> tex/quadratization.tex <==
\section{Quadratization of the power models}
\subsection{Transformation to a set of first-order ODEs}
First, we transform the models equations to a set of first-order ODEs:
%
\begin{subequations}\label{eq:en:sm:first:order:ode}
	\begin{align}
	\label{eq:en:sm:first:order:ode:delta}
	\dot \delta_i &= \omega_i, & i &= 1, \ldots, n, \\
	%
	\label{eq:en:sm:first:order:ode:omega}
	\dot \omega_i &= -\frac{D_i}{2J_i} \omega + \frac{\omega_R}{2J_i} F_i + \frac{\omega_R}{2J_i} f_i, & i &= 1, \ldots, n
	\end{align}
\end{subequations}

\subsection{Transformation to a quadratic model}
Next, we introduce the additional variables
%
\begin{subequations}
	\begin{align}
	s_i &= \sin(\delta_i), & i &= 1, \ldots, n, \\
	c_i &= \cos(\delta_i), & i &= 1, \ldots, n,
	\end{align}
\end{subequations}
%
and rewrite the nonlinear term \eqref{eq:en:sm:non:linear} in quadratic form using trigonometric identities:
%
\begin{align}\label{eq:en:sm:non:linear:quadratic}
f_i
&= -\sum_{\substack{j=1\\j\neq i}}^n K_{i,j} \sin\left(\delta_i - \delta_j - \gamma_{i, j}\right) \nonumber \\
&= -\sum_{\substack{j=1\\j\neq i}}^n K_{i,j}\Bigg[\sin(\delta_i - \delta_j)\cos(\gamma_{i, j}) - \cos(\delta_i - \delta_j)\sin(\gamma_{i, j})\Bigg] \nonumber \\
&= -\sum_{\substack{j=1\\j\neq i}}^n K_{i,j}\Bigg[\Big(\sin(\delta_i)\cos(\delta_j) - \cos(\delta_i)\sin(\delta_j)\Big)\cos(\gamma_{i, j}) \nonumber \\
&\phantom{={ }} -\Big(\cos(\delta_i)\cos(\delta_j) + \sin(\delta_i)\sin(\delta_j)\Big)\sin(\gamma_{i, j})\Bigg] \nonumber \\
&= -\sum_{\substack{j=1\\j\neq i}}^n K_{i,j}\Big[(s_i c_j - c_i s_j)\cos(\gamma_{i, j}) - (c_i c_j + s_i s_j)\sin(\gamma_{i, j})\Big], \nonumber \\
&= \sum_{\substack{j=1\\j\neq i}}^n \Big[-K_{i, j}\cos(\gamma_{i, j}) s_i c_j + K_{i, j}\cos(\gamma_{i, j}) c_i s_j \nonumber \\
&\phantom{={ }} + K_{i, j}\sin(\gamma_{i, j}) c_i c_j + K_{i, j}\sin(\gamma_{i, j}) s_i s_j\Big]
\end{align}
%
The model equations for the new variables are
%
\begin{subequations}\label{eq:en:sm:trig:variables}
	\begin{align}
	\dot s_i
	&= \cos(\delta_i) \dot \delta_i \nonumber \\
	&= c_i \omega_i, & i &= 1, \ldots, n, \\
	%
	\dot c_i
	&= -\sin(\delta_i) \dot \delta_i \nonumber \\
	&= -s_i \omega_i, & i &= 1, \ldots, n.
	\end{align}
\end{subequations}

Next, we formulate the augmented model equations, \eqref{eq:en:sm:first:order:ode} and \eqref{eq:en:sm:trig:variables}, in the quadratic form \eqref{eq:quadratic:model}, i.e., we describe the matrices $A$, $H$, and $B$. We identify that 1) the first terms on the right-hand sides of \eqref{eq:en:sm:first:order:ode} are linear in the states, 2) the second term in \eqref{eq:en:sm:first:order:ode:omega} is related to the inputs, and all terms in the nonlinear function \eqref{eq:en:sm:non:linear} are quadratic in the states.

\subsection{Matrix form}
We describe each block of the system matrices in \eqref{eq:quadratic:model}, i.e., each block in
%
\begin{subequations}\label{eq:system:matrix:blocks}
	\begin{align}
	A &=
	\begin{bmatrix}
	A_{1, 1} & \cdots & A_{1, 4} \\
	\vdots & \ddots & \vdots \\
	A_{4, 1} & \cdots & A_{4, 4}
	\end{bmatrix}, \\
	%
	H &= 
	\begin{bmatrix}
	H_{1, 1} & \cdots & H_{1, 4} \\
	\vdots & \ddots & \vdots \\
	H_{4, 1} & \cdots & H_{4, 4}
	\end{bmatrix}, \\
	%
	B &=
	\begin{bmatrix}
	B_1 \\
	\vdots \\
	B_4
	\end{bmatrix},
	\end{align}
\end{subequations}
%
where $A_{i, j}, H_{i, j}\in\mathbb R^{n\times n}$ and $B_i\in\mathbb R^{n\times m}$.

The nonzero blocks in $A$ are
%
\begin{subequations}
	\begin{align}
	A_{1, 2} &= \mathrm{I}, \\
	A_{2, 2} &= -\frac{1}{2}J^{-1}D,
	\end{align}
\end{subequations}
%
where
%
\begin{subequations}
	\begin{align}
	J &= \diag \{J_i\}_{i=1}^n, \\
	D &= \diag \{D_i\}_{i=1}^n.
	\end{align}
\end{subequations}

The Hessian, $H$, is not unique because the Kronecker product $x\otimes x$ contains duplicate elements, i.e., the product $x_i x_j$ occurs twice for $i \neq j$. It is possible to construct a symmetric Hessian, i.e. a Hessian for which $H (v\otimes u) = H (u\otimes v)$, which results in the same dynamical system as one with an asymmetric Hessian \cite{morBenB15}. We choose a Hessian with the following nonzero blocks:
%
\begin{subequations}
	\begin{align}
	H_{2, 3} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & \frac{\omega_R}{2J_i} h_i^s & -\frac{\omega_R}{2J_i} h_i^c \end{bmatrix}\right\}_{i=1}^n, \\
	H_{2, 4} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & \frac{\omega_R}{2J_i} h_i^c & \phantom{-}\frac{\omega_R}{2J_i} h_i^s \end{bmatrix}\right\}_{i=1}^n \\
	H_{3, 4} &= \blkdiag\left\{\begin{bmatrix} 0 & -e_i & 0 & 0 \end{bmatrix}\right\}_{i=1}^n, \\
	H_{4, 3} &= \blkdiag\left\{\begin{bmatrix} 0 & \phantom{-}e_i & 0 & 0 \end{bmatrix}\right\}_{i=1}^n.
	\end{align}
\end{subequations}
%
$e_i\in\mathbb R^n$ is a vector where the $i$th element is one, and all other elements are zero. The elements of the row vectors $h_i^s, h_i^c\in\mathbb R^n$ are
%
\begin{subequations}
	\begin{align}
	h_{i, j}^s &=
	\begin{cases}
	K_{i, j}\sin(\gamma_{i, j}), & j \neq i, \\
	0,                           & j =    i,
	\end{cases} \\
	h_{i, j}^c &= 
	\begin{cases}
	K_{i, j}\cos(\gamma_{i, j}), & j \neq i, \\
	0,                           & j = i.
	\end{cases}
	\end{align}
\end{subequations}

Finally, the nonzero block of $B$ is
%
\begin{align}
B_2 &= F,
\end{align}
%
where the $i$th element of $F$ is $F_i$.


==> tex/quadratization_sp.tex <==
\textbf{WARNING: THE FOLLOWING DERIVATION DOES \emph{NOT} LEAD TO A QUADRATIC MODEL, BUT RATHER TO 1) A CUBIC MODEL OR 2) A QUADRATIC DIFFERENTIAL-ALGEBRAIC MODEL}

As for the EN and the SM models, we transform the model equations to a set of first-order ODEs:
%
\begin{subequations}
	\begin{align}
	\dot \delta_i &= \omega_i, & i &= 1, \ldots, n_g, \\
	\dot \delta_i &= \frac{\omega_R}{D_i} F_i + \frac{\omega_R}{D_i} f_i, & i &= n_g+1, \ldots, n, \\
	\dot \omega_i &= -\frac{D_i}{2J_i} \omega_i + \frac{\omega_R}{2J_i} F_i + \frac{\omega_R}{2J_i} f_i, & i &= 1, \ldots, n_g.
	\end{align}
\end{subequations}
%
Again, we introduce the variables
%
\begin{subequations}
	\begin{align}
	s_i &= \sin(\delta_i), & i &= 1, \ldots, n, \\
	c_i &= \cos(\delta_i), & i &= 1, \ldots, n,
	\end{align}
\end{subequations}
%
and rewrite the nonlinear terms \eqref{eq:sp:non:linear} using trigonometric identities, i.e.,
%
\begin{align}
f_i
&= -K_{i, i+n_g}\sin(\delta_i - \delta_{i+n_g}) \nonumber \\
&= -K_{i, i+n_g}\Big[\sin(\delta_i)\cos(\delta_{i+n_g}) - \cos(\delta_i)\sin(\delta_{i+n_g})\Big] \nonumber \\
&= -K_{i, i+n_g}\Big[s_i c_{i+n_g} - c_i s_{i+n_g}\Big] \nonumber \\
&= -K_{i, i+n_g} s_i c_{i+n_g} + K_{i, i+n_g} c_i s_{i+n_g}, & i &= 1, \ldots, n_g,
\end{align}
%
and
%
\begin{align}
f_i
&= -\sum_{\substack{j=n_g+1\\j\neq i}}^n K_{i, j} \sin(\delta_i - \delta_j - \gamma_{i, j}) \nonumber \\
&= -\sum_{\substack{j=n_g+1\\j\neq i}}^n K_{i, j}\Bigg[\sin(\delta_i - \delta_j)\cos(\gamma_{i, j}) - \cos(\delta_i - \delta_j)\sin(\gamma_{i, j})\Bigg] \nonumber \\
&= -\sum_{\substack{j=n_g+1\\j\neq i}}^n K_{i, j}\Bigg[\Big(\sin(\delta_i)\cos(\delta_j) - \cos(\delta_i)\sin(\delta_j)\Big)\cos(\gamma_{i, j}) \nonumber \\
&\phantom{={ }}- \Big(\cos(\delta_i)\cos(\delta_j) - \sin(\delta_i)\sin(\delta_j)\Big)\sin(\gamma_{i, j})\Bigg] \nonumber \\
&= -\sum_{\substack{j=n_g+1\\j\neq i}}^n K_{i, j}\Bigg[\Big(s_i c_j - c_i s_j\Big)\cos(\gamma_{i, j}) - \Big(c_i c_j + s_i s_j\Big)\sin(\gamma_{i, j})\Bigg] \nonumber \\
&= \sum_{\substack{j=n_g+1\\j\neq i}}^n \Bigg[-K_{i, j}\cos(\gamma_{i, j}) s_i c_j + K_{i, j}\cos(\gamma_{i, j}) c_i s_j \nonumber \\
&\phantom{={ }} + K_{i, j}\sin(\gamma_{i, j}) c_i c_j + K_{i, j}\sin(\gamma_{i, j}) s_i s_j\Bigg],
\end{align}
%
for $i = n_g+1, \ldots, n$.

\subsubsection{Matrix form}
Again, we describe each block of the matrices $A$, $H$, and $B$ in \eqref{eq:system:matrix:blocks} separately. For the SP model, $A_{i, j}\in\mathbb R^{\bar n_i\times \bar n_j}$ and $H_{i, j}\in\mathbb R^{\bar n_i\times \bar m_j}$ where
%
\begin{subequations}
  \begin{align}
  \bar n_i &=
    \begin{cases}
    n   & i\in\{1, 3, 4\}, \\
    n_g & i = 2,
    \end{cases}\\
  %
  \bar m_j &=
    \begin{cases}
      n(3n + n_g)   & j\in\{1, 3, 4\}, \\
      n_g(3n + n_g) & j=2
    \end{cases}
  \end{align}
\end{subequations}

The nonzero blocks in $A$ are
%
\begin{subequations}
	\begin{align}
	A_{1, 2} &= \blkdiag\{\mathrm{I}, 0\}, \\
	A_{2, 2} &= -\frac{1}{2}\bar J^{-1} \bar D,
	\end{align}
\end{subequations}
%
where $I\in\mathbb R^{n_g\times n_g}$ is the identity matrix, and the $0$ denotes an $n - n_g\times n - n_g$ matrix of all zeros. The matrices $\bar J$ and $\bar D$ are
%
\begin{subequations}
	\begin{align}
	\bar J &= \diag\{J_i\}_{i=1}^{n_g}, \\
	\bar D &= \diag\{D_i\}_{i=1}^{n_g}.
	\end{align}
\end{subequations}

The nonzero blocks in the Hessian are
%
\begin{subequations}
  \begin{align}
    H_{1, 3} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & \phantom{-}\frac{\omega_R}{D_i}  h_i^s & -\frac{\omega_R}{D_i}  h_i^c\end{bmatrix}\right\}_{i=1}^n,     \\
    H_{1, 4} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & \phantom{-}\frac{\omega_R}{D_i}  h_i^c & \phantom{-}\frac{\omega_R}{D_i}  h_i^s \end{bmatrix}\right\}_{i=1}^n,     \\
    H_{2, 3} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & 0 & -\frac{\omega_R}{2J_i} h_i \end{bmatrix}\right\}_{i=1}^{n_g}, \\
    H_{2, 4} &= \blkdiag\left\{\begin{bmatrix} 0 & 0 & \frac{\omega_R}{2J_i} h_i & 0 \end{bmatrix}\right\}_{i=1}^{n_g}, \\
    H_{3, 4} &= \blkdiag\{\begin{bmatrix} 0 & \phantom{-}e_i & 0 & 0 \end{bmatrix}\}_{i=1}^n, \\
    H_{4, 3} &= \blkdiag\{\begin{bmatrix} 0 & -e_i           & 0 & 0 \end{bmatrix}\}_{i=1}^n,
  \end{align}
\end{subequations}
%
where $e_i\in\mathbb R^{n_g}$ is a row unit vector, and the elements of the row vectors $h_i, h_i^s, h_i^c\in\mathbb R^n$ are
%
\begin{subequations}
  \begin{align}
    h_{i, j} &=
    \begin{cases}
      K_{i, j}, & i\in\{1, \ldots, n_g\}, \quad j = i + n_g, \\
      0,         & \mathrm{otherwise},
    \end{cases} \\
    %
    h_{i, j}^s &=
    \begin{cases}
      K_{i, j}\sin(\gamma_{i, j}), & i\in\{n_{g+1}, \ldots, n\},   \quad j\in\{n_{g+1}, \ldots, n\}\backslash\{i\}, \\
      0,                           & \mathrm{otherwise},
    \end{cases} \\
    %
    h_{i, j}^c &=
    \begin{cases}
      K_{i, j}\cos(\gamma_{i, j}), & i\in\{n_{g+1}, \ldots, n\},   \quad j\in\{n_{g+1}, \ldots, n\}\backslash\{i\} \\
      0,                           & \mathrm{otherwise},
    \end{cases} 
  \end{align}
\end{subequations}

